Kinematic Wave Models of Network Vehicular Traffic

The kinematic wave theory, originally proposed by (Lighthill and Whitham, 1955b; Richards, 1956), has been a good candidate for studying vehicular traffic. In this dissertation, we study kinematic wave models of network traffic, which are expected to be theoretically rigorous, numerically reliable, and computationally efficient. For traffic systems with inhomogeneous links, merges, diverges, or mixed-type vehicles, we study the kinematic waves in their Riemann solutions and develop numerical solution methods of the Godunov type and the supply-demand type. For a network traffic system, we propose a multi-commodity kinematic wave (MCKW) model and an implementation of it. The model observes First-In-First-Out principle in the order of a time interval and is numerically convergent. Further, we apply this simulation model to study equilibrium states and periodic waves in road networks. Finally, we summarize our work and discuss future research directions.

==> conclusion/4th_conc.tex <==
\section{Experimental and theoretical investigations of traffic flow at
highway merges: A proposal}
\subsection{Background}
Everyday traffic congestion can be caused by many factors, such as
traffic accidents, bad weather and highway (geometric)
bottlenecks. Among highway bottlenecks, it is well recognized that
merges, where two or more streams of traffic merge into one, such as
at a freeway on-ramp or freeway to freeway junction, are often the
locations where congestion initiates.  A regular traveler of a
freeway can easily tell you these congestion spots. Two examples
that the author is familiar with are the I-80 and Business 80 merge
at the west side of Sacramento and the I-5 and 405 merge near El
Toro (the notorious El Toro Y which is known for its heavy
congestion during evening peak hours) in Orange County.   Two often
used measures to improve traffic conditions at problematic merging
junctions are geometric improvement (such as adding lanes to the
downstream branch) and  traffic control (such as ramp or freeway to
freeway metering), both  require a good understanding  of traffic flow
behavior for their  successful applications.   A better understanding 
of
traffic behavior at merges  therefore allows for more streamlined
geometric design of merges, and more efficient  ramp control
\citep{chen1997metering,papageorgiou1997ALINEA}.  Moreover, merges are also
building blocks of road networks. A sound merge model is an essential
element of any network traffic flow model.

Because of these important roles that merges play in a road
network, many studies have been devoted to model traffic flow at
merges 
\citep{kerner1996complexity,kerner1996jams,daganzo1999remarks, 
cassidy1999bottlenecks,kita1999merging,daganzo1995ctm,lebacque1996godunov,jin2003merge}, in which
various approaches were explored.  In one approach, traffic
dynamics was simulated with microscopic traffic flow
models \citep{kita1999merging}, in which a set of
merging rules are imposed on individual merging vehicles. Although
this kind of models provide a detailed description of merging
behavior of individual vehicles, the merging behavior itself is not
yet well understood largely because realistic data to test various
behavior hypotheses are not available up to now.  In another
approach, traffic dynamics at merges was modeled at a macroscopic
level.  In one type of macroscopic merge models, the effects of an
entry ramp on highway traffic were captured through a `momentum
change' to highway traffic \citep{kunhe1992continuum, kerner1995jams,
helbing1998kinetic,lee2000onramp}. In another type, traffic dynamics at a
merge was studied using the so-called supply-demand
method \citep{daganzo1995ctm,lebacque1996godunov,jin2003merge}, in which the
amount of traffic through the merge is decided by the supply of the
downstream branch and the demands of the upstream merging
branches.

In the first type of macroscopic merge models, only the effect
of  on-ramp traffic to highway traffic has been considered.
However,  this is not enough to
consider dynamics of a merge, for which the interaction between the
upstream highway and the on-ramp has to be taken into account, since,
at merges, congestion on one branch may cause congestion on another.
Observing a typical merge with one upstream freeway and an on-ramp,
for example, a very long queue on the on-ramp may slow down traffic
flow on the upstream freeway and after sometime traffic on the
upstream freeway becomes congested; on the other hand, when the
upstream freeway is highly congested, even a few vehicles from the
on-ramp may have to wait for a long time to squeeze in. Nevertheless,
this is not a problem for the supply-demand merge models. Therefore, 
to use
the first or second type of macroscopic merge models depends on 
whether we are
interested in dynamics of only the highway or both.

Regardless of which merge model we adopt in an application, we
face the same problem---we do not know how realistic it is
in  describing real traffic at merges, because none of the merge
models have been carefully validated under real driving
conditions. Considering the important role merges play in shaping
network traffic flow evolution, it is highly desirable to gain a
thorough understanding of how traffic flow through a merge evolves,
and this can only be done through a systematic study of traffic data
collected at merges.

\subsection{Proposed research and research methodology}

In this research, we propose to utilize the  PEMS database, which
stores traffic flow data from many California freeways,  to
study  traffic flow patterns at merges and use the experimental
findings  to check the validity of various assumptions adopted in 
macroscopic merging
models.  We will consider two types of merges in this study---ramp to
freeway merges and freeway to freeway merges, because we suspect
that traffic behavior at the two types of merges  may be different.
For one, at ramp to freeway merges ramp traffic has lower priority
in obtaining right-of-way and has to find acceptable gaps for safe
merging.  Thus data for both types of merges will be collected and
studied.

Our major interest in merge traffic is the possible traffic flow
patterns (or states) that exist at a merge.  Because many
combinations of dynamic states can appear at a  merge, it is not easy
to understand the properties of merging traffic flow with transient
states. However, if the traffic states of all  branches close to the
merge do not change for a period of time (\textit{stationary states}),
their properties can be revealed more easily.   In fact, the 
importance
of stationary states to the dynamics of  merging traffic was first
realized by \cite{daganzo1996gridlock}.  When considering a merge
with an upstream highway and an on-ramp, Daganzo suggested that
only the following four types of stationary states can  exist: No Q 
(all
branches are free-flow), Ramp Q (the  on-ramp is
congested, the upstream highway is free-flow, the  downstream
highway congested or at capacity flow),  Highway  Q (the upstream
highway  congested, the on-ramp free-flow, the downstream
highway  congested or at capacity flow), Both Q (all branches are
congested or at capacity flow). Although these conjectures are quite
intuitive, they still need to be validated with experimental
observations.

After studying the morning peak traffic dynamics at the merge of the 
Queen Elizabeth Way (QEW) and Cawthra Road in  
metropolitan Toronto, Canada, 
\cite{cassidy1999bottlenecks} found an active bottleneck, starting from the 
merging point and ending at about 810 meters downstream, and the 
total inflow from the upstream highway and the on-ramp is the same as 
the outflow from the bottleneck. Omitting the dynamics in the 
bottleneck, we can see that this is a stationary state. It is also 
reported that the stationary state is consistent from day to day. 
However, it is shown that the discharge rate, known as the bottleneck 
capacity \citep{banks1991metering, hall1991capacity}, is lower than 
the capacity flow-rate of the downstream link when the bottleneck is
not active (8 percent lower in \cite{cassidy1999bottlenecks}; less than 10 
percent lower  in
\cite{banks1991metering}). Although these observations present a
challenge to  the models using the supply-demand method 
\citep{daganzo1995ctm,lebacque1996godunov,jin2003merge}, in which the
discharge flow  is considered to be the supply of the downstream link
(the capacity  flow in this case), we may first examine the validity of
the supply-demand method under one-capacity situations and then
find ways to extend the supply-demand method to address
the so-called  two-capacity phenomena at merges.   In
\cite{cassidy1999bottlenecks},  the inflow of the upstream link and the on-ramp
is combined together  since traffic dynamics of the upstream freeway and on-ramp were not of interest. However, to study the distribution of  the discharge rate between the upstream
links as well as  the  queueing process in the upstream
links, we need to study link-specific flow data at least 800 meters 
upstream to the merging point (this requirement is more relevant
to freeway to freeway merges). Note that the outflow and the 
corresponding occupancy should be measured at a point at least 
2,500 ft downstream the merging point, which is consistent with the 
distance given in the definition of capacity by HCM 
(1985)\nocite{hcm1985}.  Otherwise,  traffic flow can have large
oscillations  between the merge and the measurement point \citep{urbanikii1991evaluation}, and stationary states can hardly be observed at the
measurement locations. 

To get a clearer picture of the underlying relations between
stationary states at merges, we will choose to study isolated
merges, in particular those without the presence of significant
immediate upstream/downstream  diverges, so as to avoid the
complications arising from interactions between merges and
diverges.  The data we shall extract from the PEMS database are flow 
and occupancy at all branches of a merge.  Another possible source of
data is the trajectories extracted  from the video data
\citep{coifman1997shock}, but still we will focus on  the aggregate-level
information, e.g. the number of vehicles in a  section of highway or
on-ramp.  

To identify stationary states from flow-rates, occupancies,
and/or  velocities in time series, we apply low-pass filtering, such as
the  cumulative curve approach used in \cite{cassidy1999bottlenecks}. If the
inflow  and outflow of a merge are nearly equal to each other for a
certain amount of time, say at least 15 minutes (the specific time
length can be further investigated), or the number of vehicles in the
bottleneck downstream of a  merge is nearly constant, we will
consider the corresponding traffic  states as stationary. Our study will
first identify, from a large  amount of data collected at certain
merges, all possible combinations of stationary states  existing in
these merges. Stationary states will be categorized into recurrent 
and non-recurrent, according to whether they appear from day to
day  or not. Besides stationary states in congested peak hours, we
will also be  interested in those in free flow. 

Note that stationary states are defined in the average sense. Thus
statistical properties of each set  of stationary states will also be
studied. With identified stationary  states, we can then simplify
traffic dynamics as a combination of  stationary states,  plus the
corresponding intermediate states.  After obtaining the stationary
states at the selected merges, Daganzo's conjectures can then be
checked. Moreover, the obtained stationary states also allow us to
validate the assumptions adopted in macroscopic merge models,
including the definitions of traffic supply, demand and capacity at a
merge because, if a merge model is any good, it should at least be
able to reproduce the stationary states. 

As to the further investigation of macroscopic merge models, we
are particularly interested in validating their distribution schemes.
Distribution schemes play the role of allocating the total amount of
flow through a merge into its contributing upstream branches. Three
distribution schemes have been suggested in literature
\citep{daganzo1995ctm,lebacque1996godunov,jin2003merge}.  With observed sets
of stationary states, we'll able to check the validity of
these distribution schemes, which to a large degree also
validate these merge models. With a validated and well calibrated
merge model, we can then reproduce transient states at merges under
different initial/boundary conditions, and compare these model
predictions with experimental observations. Note that, in these 
models, we can simply use the bottleneck capacity as the downstream 
supply. However, it will be an interesting problem to address the 
two-capacity phenomena in the kinematic wave models. 

The proposed investigations on merges, we hope, would lead to a
better understanding of merging traffic dynamics, a definitive 
classification of
stationary states, and an in-depth study of macroscopic merge
models. Progress made in all these areas would in turn lead to more
effective geometric improvements and ramp or freeway to freeway
metering [e.g. \citep{banks1991metering}] to reduce congestion at 
problematic merge locations.

\subsection{Work Tasks}
\begin{enumerate}
\item Selection of merge sites

\item Extracting and processing traffic data from the PEMS database

\item Identification and classification of stationary states

\item Validation of macroscopic merge models

\item Study of transient states and merge flow dynamics
\item Prepare final report

\end{enumerate}

\subsection{Expected results and products}
This research is expected to 1)  help
us understand the flow patterns at merges,  2) validate and calibrate
macroscopic merge models, and 3) enhance our ability to improve
traffic conditions at merges.

The main product of this research will be findings about traffic
behavior at merges and models that describe it.


